Properties of UTxO Ledgers and Programs Implemented on Them

Trace-based properties are the gold standard for program behaviour analysis. One of the domains of application of this type of analysis is cryptocurrency ledgers, both for the purpose of analyzing the behaviour of the ledger itself, and any user-defined programs called by it, known as smart contracts. The (extended) UTxO ledger model is a kind of ledger model where all smart contract code is stateless, and additional work must be done to model stateful programs. We formalize the application of trace-based analysis to UTxO ledgers and contracts, expressing it in the languages of topology, as well as graph and category theory. To describe valid traces of UTxO ledger executions, and their relation to the behaviour of stateful programs implemented on the ledger, we define a category of simple graphs, infinite paths in which form an ultra-metric space. Maps in this category are arbitrary partial sieve-define homomorphisms of simple graphs. Programs implemented on the ledger correspond to non-expanding maps out of the graph of valid UTxO execution traces. We reason about safety properties in this framework, and prove properties of valid UTxO ledger traces.

==> 0_Abstract/Polina_abstract.tex <==
\begin{abstract}

 Trace-based properties are the gold standard for program behaviour analysis.  One of the domains of application of this type of analysis is cryptocurrency ledgers, both for the purpose of analyzing the behaviour of the ledger itself, and any user-defined programs called by it, known as smart contracts.   There is also a robust tradition of using category theory to model ledgers, in particular, UTxO-style ledgers, which consider in this work. Underlying our   analysis is a ledger model, as well as a smart contract implementation model, expressed in terms of small-step semantics. We describe valid traces of UTxO ledger executions, and their relation to the behaviour of stateful programs implemented on the ledger, in category-theoretic terms. Specifically, we define a category of simple   graphs, infinite paths in which form an ultrametric space. Maps in this category are arbitrary partial sieve-define homomorphisms of simple graphs. Programs implemented on the ledger, as well as ledger properties expressed in the same framework, define non-expanding maps out of the graph of valid UTxO execution traces. We prove certain properties of   valid UTxO ledger traces.


  % The specifics of smart contract-enabled UTxO (EUTxO) ledger design allow us to
  % construct a categories related to execution graphs, one of which includes directed
  % graphs representing
  % sequences of ledger states resulting from valid updates. The other category contains
  % simple graphs where the vertices are labelled with the transition input as well as
  % a start state. We demonstrate that the former lifts to the latter, and
  % also forms an ultra-metric space. We define a subsets of properties of paths in
  % the execution graphs that are better suited to represent notions of safety
  % and liveness in blockchain executions, as they exclude reasoning about unreachable
  % ledger states, which is a relevant distinction for EUTxO programming. We demonstrate
  % when these classes of properties of stateful contracts can be
  % guaranteed by their ledger
  % implementations. We present examples of ledger properties in our framework, and how
  % to use the simulation relation between graphs to we present to express them.
  %
  %   Smart contract-enabled cryptocurrency ledgers are designed to support execution of
  %   user-defined code as part of transaction processing. Many common smart
  %   contracts can be viewed as \emph{stateful} by considering a specially identified
  %   subsection of records on the ledger as the contract state, e.g. the set of DEX
  %   offers, the total quantity of a particular type of asses, set of bids in
  %   an auction, etc. The structured contract framework, introduced in \cite{structured},
  %   formalizes the notion of correctly implemented stateful contracts for ledgers
  %   whose evolution can be specified using small-step semantics.
  %   In this work, we specify what it means for a contract
  %   or ledger \emph{execution trace} to be \emph{valid}, expressed in terms of its
  %   specification and some initial conditions.
  %
  %   Next, we show that definitions of
  %   liveness and safety properties, as presented in \cite{liveness}, can be adapted
  %   to the space of valid execution traces for both ledger and contract traces.
  %   This allows us to derive a result similar to the one given in \cite{liveness},
  %   characterizing all properties via liveness and safety.
  %   We then show that under certain constraints on ledger and contract initial
  %   conditions, we can construct a total, continuous map from ledger traces to
  %   traces of a specific structured contract. We prove that this map can be used
  %   to lift safety properties of contract traces to safety properties of ledger
  %   traces. We also show that liveness properties at the ledger level map onto
  %   liveness properties of the contract, and, moreover, when the map is surjective,
  %   the preimages of liveness properties are also liveness properties.
  %
  %   %\
  %   keywords

    {blockchain  \and ledger \and smart contract \and formal verification \and
    specification \and transition system \and UTxO \and properties \and liveness \and safety}
\end{abstract}


==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Cynthia Kop and Helida Salles Santos (Eds); 19th Workshop on\\ Logical and Semantic Frameworks with Applications (LSFA'24)\\
EPTCS 421, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.421.1}{10.4204/EPTCS.421.1}}

